Stabilizing reinforcement learning control: A modular framework for optimizing over all stable behavior

We propose a framework for the design of feedback controllers that combines the optimization-driven and model-free advantages of deep reinforcement learning with the stability guarantees provided by using the Youla-Kucera parameterization to define the search domain. Recent advances in behavioral systems allow us to construct a data-driven internal model; this enables an alternative realization of the Youla-Kucera parameterization based entirely on input-output exploration data. Perhaps of independent interest, we formulate and analyze the stability of such data-driven models in the presence of noise. The Youla-Kucera approach requires a stable "parameter" for controller design. For the training of reinforcement learning agents, the set of all stable linear operators is given explicitly through a matrix factorization approach. Moreover, a nonlinear extension is given using a neural network to express a parameterized set of stable operators, which enables seamless integration with standard deep learning libraries. Finally, we show how these ideas can also be applied to tune fixed-structure controllers.

==> sections/tank-control-long.tex <==

\subsection{An industrial example}
\label{subsec:extank}






For the next example, we incorporate nonlinearity and integral action into the setup. The environment is a nonlinear two-tank system whose level and inflow rate are controlled by \ac{PID} controllers. Unlike prior works that use \ac{RL} to adjust the \ac{PID} parameters, we augment \iac{PID} controller with the proposed stabilizing framework.  \par
The problem involves controlling the liquid level in an upper tank, positioned vertically above a second tank that serves as a reservoir. Water drains from the tank into the reservoir through an outflow pipe, and is replenished by water from the reservoir delivered by a pump whose flow rate is our manipulated variable. More precisely, two \ac{PID} controllers are in operation: 
the ``level controller''
%Given the desired level, one \ac{PID} controller 
outputs the desired flow rate based on level tracking error,
and the ``flow controller'' uses the requested flow rate as a reference signal  to set the pump speed.
{\color{blue}
System parameters, values, and descriptions are given\footnote%
{\color{blue}2023-08-19 [PDL]: The table has disappeared. We could
either restore it, or find a deft way simply to cite it. Suggestions?} 
in \cref{table:tank}.
}\par



 % Significant physical dimensions include
% $r_{\text{tank}}$, the radius of the top tank;
% $r_{\text{pipe}}$, the radius of the pipe for the outflow of the top tank; and
% $\ell$, the distance from the base of the top tank up to the water surface.
% (We later refer to $m$, a filtered counterpart of $\ell$.)

% Key flow parameters, with units of volume/time,
% are the outflow $f_{\text{out}}$;
% the inflow $f_{\text{in}}$;
% an empirical coefficient $f_c$;
% and $f_{\text{max}}$, the maximum flow the pump can deliver.\par
% The pump delivers water to the top tank at the rate
% $(p/100)f_{\rm max}$,
% where $p$ is a dimensionless percentage in $[0,100]$.

% We write $\bar{p}$ for the commanded pump speed,
% typically a piecewise-constant setpoint function.

\begin{figure}[tbp]
\begin{center}
\includegraphics[width=8.4cm]{rewards_median_quant_2.pdf}    % The printed column width is 8.4 cm.
\caption{Cumulative reward curve over $20$ training sessions. The solid line is the median and the shaded region shows the interquartile range. The dashed line and its shaded region are the final results of training without the stability constraint.} 
\label{fig:rewards_tank}
\end{center}
\end{figure}

\emph{(System description)}\quad
The system dynamics are based on Bernoulli's equation, $f_{\text{out}}\approx f_c\sqrt{2 g\ell}$, and the conservation of fluid volume in the upper tank:
\begin{equation}
\frac{d\hfil}{dt}\left(\pi r_{\text{tank}}^2\ell\right)
= \pi r_{\text{tank}}^{2} \dot\ell
= f_{\text{in}} - f_{\text{out}}.
\end{equation}
(We use dot notation to represent differentiation with respect to time.)
% Our system model combines the principles above with some simple filters to make our mathematical description physically realizable. A first-order filter with time constant $\tau\ge0$
% transforms an input signal $\hat{y}$
% into the output signal $y$ defined by
% \begin{equation}
% \tau \dot{y} + y = \hat{y},
% \qquad y(0)=0.
% \end{equation}
% Note that setting $\tau=0$ gives $y(t)=\hat y(t)$, while if $\hat y$ is constant,
% one has $y(t) = (1 - e^{-t/\tau})\hat y$.
Our application involves four filtered signals with time constants
$\tau_p$ for the pump,
$\tau_{\text{in}}$ for changes in the inflow,
$\tau_{\text{out}}$ for the outflow,  and
$\tau_m$ for the measured level dynamics. We have the following system of differential equations describing the pump, flows, level, and measured level:
\begin{align}
\tau_p \dot{p} + p &= p_{\text{sp}}\\
\tau_{\text{in}} \dot{f}_{\text{in}} + f_{\text{in}} &= f_{\text{max}} \left(\frac{p}{100}\right)\\
\tau_{\text{out}} \dot{f}_{\text{out}}+ f_{\text{out}} &= \pi r_{\text{pipe}}^{2} f_{\text{c}} \sqrt{2 g \ell}\\
\pi r_{\text{tank}}^{2} \dot{\ell} &= f_{\text{in}} -  f_{\text{out}}\\
\tau_m \dot{m} + m &= \ell
\end{align}
To track a desired level $\ell_{\text{sp}}$ --- ``sp'' stands for ``setpoint'' --- we can employ level and flow controllers by including the following equations:
\begin{align}
\begin{split}
p_{\text{sp}} &= \text{PID}_{\text{flow}} (f_{\text{in,sp}} - f_{\text{in}}) \\
f_{\text{in,sp}} &= \text{PID}_{\text{level}}(\ell_{\text{sp}} - m)
\label{eq:PIDtank}
\end{split}
\end{align}

Equation~\eqref{eq:PIDtank} uses shorthand for \ac{PID} controllers taking the error signals $f_{\text{in,sp}} - f_{\text{in}}$ and $\ell_{\text{sp}} - m$, respectively. For our purposes, $\text{PID}_{\text{flow}}$ and $\text{PID}_{\text{level}}$ are fixed and a part of the environment. 
These dynamics are implemented in discrete time steps of $0.5$ seconds and with Gaussian measurement noise with variance $0.015$.\par

%\begin{figure}[tbp]
%\begin{center}
%\includegraphics[width=8.4cm]{heatmap_output_2.pdf}    % The printed column width is 8.4 cm.
%\caption{A global view of the training progress across all $20$ sessions. For each episode, a distribution of time spent at various output values is obtained. The heatmap shows the average amount of time spent at each episode--output coordinate.} 
%\label{fig:heatmap_output}
%\end{center}
%\end{figure}

%\begin{figure}[tbp]
%\begin{minipage}[]{\linewidth}
%\begin{center}
%    \sidesubfloat[]{%
%      \includegraphics[[width=8.4cm], height=0.38\textheight, keepaspectratio]{rewards_median_quant_2.pdf}\label{fig:rewards_tank}}\hfill\\
%    \sidesubfloat[]{%
%      \includegraphics[[width=8.4cm], height=0.38\textheight, keepaspectratio]{heatmap_output_2.pdf}\label{fig:heatmap_output}}\hfill\\
%\caption{(a) Cumulative reward curve over $20$ training sessions. The solid line is the median and the shaded region shows the interquartile range. The dashed line and its shaded region are the final results of training without the stability constraint.; (b) A global view of the training progress across all $20$ sessions. For each episode, a distribution of time spent at various output values is obtained. The heatmap shows the average amount of time spent at each episode--output coordinate.}
%\label{fig:ex2}
%\end{center}
%\end{minipage}
%\end{figure}


\emph{(Training results)}\quad
Since the environment includes \iac{PID} controller, we modify the control scheme to be in incremental form $u_t = u_{t-1} + \Delta u_t$, where $\Delta u_t$ is the sum of the \red{nonlinear} \ac{YK}  parameter \red{from \cref{subsec:stablenonlin}} and \ac{PID} controller outputs:
\[
\Delta u_t = \Delta u^{(q)}_t + \Delta u^{(\text{PID})}_t
\]
We ran $20$ training sessions, each of $100$ episodes.\Cref{fig:rewards_tank} illustrates the cumulative rewards observed. The median over the $20$ sessions provides the solid line; the interquartile ranges delimit the shaded region.
We note that the median reward curve is much closer to the upper limit of the shaded region than the lower, indicating that the majority of experiments fall within that tight region. Although there is significant change in the first few episodes, due to the random policy initialization, the training sessions exhibit consistent convergence. The reward curves tend to plateau after around $40$ episodes. \Cref{fig:input_output} shows a single rollout from one of the experiments. 
\par

%\Cref{fig:heatmap_output} shows the collective evolution of each episode throughout the training sessions. Each episode-output coordinate is shaded based on how much time the output variable spent there on average. Darker shading around the dashed values (setpoints) is more desirable. The purpose of this figure is to provide a rough translation of what the reward curve in \cref{fig:rewards_tank} entails. On the other hand, \cref{fig:input_output} shows a single rollout from one of the experiments. 


\begin{figure}[tbp]
\begin{center}
\includegraphics[width=8.4cm]{input_output_2.pdf}    % The printed column width is 8.4 cm.
\caption{A sample input-output rollout by the trained \ac{RL} agent for one of the training sessions. Dashed lines are setpoints; solid lines are measured values.} 
\label{fig:input_output}
\end{center}
\end{figure}

